ChemHGNN: A Hierarchical Hypergraph Neural Network for Reaction Virtual Screening and Discovery

Reaction virtual screening and discovery are fundamental challenges in chemistry and materials science, where traditional graph neural networks (GNNs) struggle to model multi-reactant interactions. In this work, we propose ChemHGNN, a hypergraph neural network (HGNN) framework that effectively captures high-order relationships in reaction networks. Unlike GNNs, which require constructing complete graphs for multi-reactant reactions, ChemHGNN naturally models multi-reactant reactions through hyperedges, enabling more expressive reaction representations. To address key challenges, such as combinatorial explosion, model collapse, and chemically invalid negative samples, we introduce a reaction center-aware negative sampling strategy (RCNS) and a hierarchical embedding approach combining molecule, reaction and hypergraph level features. Experiments on the USPTO dataset demonstrate that ChemHGNN significantly outperforms HGNN and GNN baselines, particularly in large-scale settings, while maintaining interpretability and chemical plausibility. Our work establishes HGNNs as a superior alternative to GNNs for reaction virtual screening and discovery, offering a chemically informed framework for accelerating reaction discovery.

==> 2Related_Study.tex <==
\subsection{Graph Neural Networks for Chemistry}
Graph Neural Networks (GNNs) have emerged as powerful frameworks for molecular representation learning since molecules naturally form graph structures with atoms as nodes and bonds as edges \cite{guo2023graph}. The Message Passing Neural Network framework has become foundational, where atom embeddings are iteratively updated through information exchange with neighboring atoms \cite{gilmer2017neural}. Despite their success, traditional GNNs face significant limitations when modeling multi-reactant systems, as they struggle to represent important chemical features including functional groups, spatial relationships, and multi-way interactions \cite{coley2019graph,rong2020self}.

\subsection{Hypergraph Representation of Reaction Networks}
Conventional graphs can only represent pairwise correlations, which is insufficient for modeling complex chemical systems where higher-order relationships are prevalent \cite{chen2024molecular}. Hypergraphs extend graphs to accommodate high-order correlations, making them especially suitable for representing multi-participant chemical reactions \cite{chang2024hypergraph}. Recent work has introduced chemical hypergraphs as a unified mathematical structure where metabolites serve as nodes and hybrid edges represent both metabolic directionality and high-order interactions \cite{huang2025multi}. This approach more naturally captures the inherent higher-order relationships in reaction networks, including reactant-product directionality \cite{yadati2020nhp}.

\subsection{Hyperlink Prediction}
As a natural extension of link prediction on graphs, hyperlink prediction aims to infer missing hyperlinks in hypergraphs \cite{chen2023survey}. This has direct applications in chemical reaction networks, where methods can be categorized into similarity-based, probability-based, matrix optimization-based, and deep learning-based approaches. Neural Hyperlink Predictor (NHP) adapts GCNs for link prediction in both undirected and directed hypergraphs, with NHP-D being the first method specifically designed for directed hypergraphs \cite{yadati2020nhp}. The hypergraph representation preserves reaction context and uncovers hidden insights not apparent in traditional directed graph representations \cite{mann2023ai}. Hypergraph Neural Networks have demonstrated superior performance in molecular property prediction tasks, even outperforming models that utilize 3D geometric information \cite{chen2024molecular}.
